EventPlus: A Temporal Event Understanding Pipeline

We present EventPlus, a temporal event understanding pipeline that integrates various state-of-the-art event understanding components including event trigger and type detection, event argument detection, event duration and temporal relation extraction. Event information, especially event temporal knowledge, is a type of common sense knowledge that helps people understand how stories evolve and provides predictive hints for future events. EventPlus as the first comprehensive temporal event understanding pipeline provides a convenient tool for users to quickly obtain annotations about events and their temporal information for any user-provided document. Furthermore, we show EventPlus can be easily adapted to other domains (e.g., biomedical domain). We make EventPlus publicly available to facilitate event-related information extraction and downstream applications.

==> tables/eval_biomed_cotraining.tex <==

\begin{table}[h]
    \footnotesize
    \centering
    \begin{tabular}{@{\ \ }l|@{\ \ }l|c@{\ \ }|c@{\ \ }|c@{\ \ }|c@{\ \ }}
        Corpus & Model & Trig-I & Trig-C & Arg-I & Arg-C \\ \hline
        \multirow{2}{*}{ACE} & Single & \textbf{76.67} & \textbf{72.79}  & \textbf{61.96} & \textbf{58.47} \\
        & MDT & 75.45 & 71.20  & 60.96 & 55.87 \\ \hline 
        \multirow{2}{*}{GENIA} 
        & Single & 75.78 & 71.39  & 63.51 & 63.16 \\
        & MDT & 76.28 & 71.92  & 64.47 & 64.29 \\
        &  \ftscibert{} & \textbf{78.52} & \textbf{74.66}  & \textbf{71.55} & \textbf{71.02} 
    \end{tabular}
    \caption{Model performance comparison on ACE and \genia{} dev set. The single model for ACE refers to the model described in section \ref{subsec:ee_ace}, while that for GENIA refers to the same model trained on GENIA. MDT represents the model trained on the two datasets.  }
    \label{table:co_training}
\end{table}


% \begin{table}[t]
%     % \small
%     \centering
%         \begin{tabular}{@{\ \ }l|c@{\ \ }c@{\ \ }c@{\ \ }c@{\ \ }}
%             \hline \textbf{Model} & \textbf{Trig-I}  & \textbf{Trig-C}  & \textbf{Arg-I} & \textbf{Arg-C} \\
%             \hline
            
%             Single  & 76.67 & 72.79  & 61.96 & 58.47 \\
%             \hline
%             Co-training & 75.45 & 71.20  & 60.96 & 55.87 \\
%             \hline
%         \end{tabular}
%     \caption{\label{font-table} Model performance comparison on ACE and \genia{} dev set.}
%     \label{table:co_training}
%     \vspace{-1em}
% \end{table}


% \begin{table}[t]
%     % \small
%     \centering
%         \begin{tabular}{@{\ \ }l|c@{\ \ }c@{\ \ }c@{\ \ }c@{\ \ }}
%             \hline \textbf{Model} & \textbf{Trig-I}  & \textbf{Trig-C}  & \textbf{Arg-I} & \textbf{Arg-C} \\
%             \hline
            
%             \ftscibert{}  & 78.52 & 74.66  & 71.55 & 71.02 \\
%             \hline
%             Co-training & 76.28 & 71.92  & 64.47 & 64.29 \\
%             \hline
%         \end{tabular}
%     \caption{\label{font-table} Model performance comparison on \genia{} dev set.}
%     \label{table:co_training_scibert}
%     \vspace{-1em}
% \end{table}
